A solid-state nuclear clock based on VUV absorption spectroscopy of $^{229}$Th

We demonstrate sustained operation of a solid-state thorium-229 nuclear clock using continuous-wave absorption at 148.4 nm. In a $^{229}\mathrm{Th}:\mathrm{CaF}_2$ crystal, we resolve four quadrupole components of the D center and a broader O-center resonance. Feedback on the strongest narrow component is updated approximately every 10 s and remains active throughout a 30-h record. A hydrogen-maser-referenced frequency comb measures the output. Its fractional frequency instability follows approximately $1.29\times10^{-11}(\tau/\mathrm{s})^{-1/2}$ and reaches $1.24\times10^{-13}$ at $10^4$ s. A separate 6.6-h run demonstrates feedback on a second quadrupole component. These measurements connect the resolved absorption spectra with sustained nuclear-clock operation and frequency comparisons between crystal segments.

==> generated/b_repeat_rows.tex <==
Initial run & 30.14 & 22.690 & $298\,796.17\pm0.08$ & --- \\
Repeat 1 & 3.19 & 22.506 & $298\,796.63\pm0.20$ & $+0.46\pm0.21$ \\
Overnight & 8.15 & 22.683 & $298\,797.55\pm0.19$ & $+1.38\pm0.21$ \\
Repeat 2 & 1.00 & 22.260 & $298\,797.80\pm0.38$ & $+1.63\pm0.39$ \\


==> generated/fit_rows.tex <==
$a$ & 6 & $+22.3(85)$ & $197(33)$ & $3.64(30)$ & 1.13 \\
$b$ & 5 & $+13.6(16)$ & $83(6)$ & $16.88(69)$ & 0.67 \\
$c$ & 2 & $+10.8(55)$ & $118(22)$ & $7.54(74)$ & 1.88 \\
$d$ & 3 & $-26.0(66)$ & $117(27)$ & $4.76(55)$ & 0.96 \\
$e$ & 4 & --- & $200$ (fixed) & $0$ (boundary)$^{\ddagger}$ & 1.84 \\
$O$ & 3 & $-27.0(400)$ & $893(143)$ & $4.35(35)$ & 1.37 \\


==> generated/frequency_rows.tex <==
$a$ & $285\,663(12)$ & $285\,641(9)$ & $285\,662(5)$ & $+22.3\pm14.7$ & $+1.3\pm12.7$ & $+7.1\pm16.7$ & $-36.5\pm18.8$ \\
$b_{\rm scan}$ & $298\,795.6(16)$ & $298\,782(4)$ & $298\,784(5)$ & $+13.6\pm4.3$ & $+11.6\pm5.2$ & $+11.6\pm4.4$ & $+6.6\pm5.6$ \\
$c_{\rm scan}$ & $444\,530.8(55)$ & $444\,520(5)$ & $444\,551(3)$ & $+10.8\pm7.4$ & $-20.2\pm6.3$ & $+31.8\pm13.1$ & $+32.2\pm20.3$ \\
$d$ & $528\,977.0(66)$ & $529\,003(14)$ & $529\,021(3)$ & $-26.0\pm15.5$ & $-44.0\pm7.2$ & $-8.7\pm17.8$ & $-0.8\pm17.4$ \\
$b_{\rm clock}$ & $298\,796.17(13)$ & $298\,782(4)$ & $298\,784(5)$ & $+14.2\pm4.0$ & $+12.2\pm5.0$ & $+12.2\pm4.1$ & $+7.2\pm5.3$ \\
$c_{\rm clock}$ & $444\,524.78(91)$ & $444\,520(5)$ & $444\,551(3)$ & $+4.8\pm5.1$ & $-26.2\pm3.1$ & $+25.8\pm11.9$ & $+26.2\pm19.5$ \\


==> generated/scan_consistency_rows.tex <==
$a$ & 6 & $+22.1\pm7.4$ & $5.62/5$ \\
$b$ & 5 & $+13.4\pm1.6$ & $2.93/4$ \\
$c$ & 2 & $+12.0\pm5.3$ & $0.04/1$ \\
$d$ & 3 & $-28.5\pm6.5$ & $1.70/2$ \\
$O$ & 3 & $-60.1\pm34.1$ & $3.21/2$ \\


==> generated/temperature_rows.tex <==
$a$ & $13.300$ & $+15.162$ & $+37.772$ & $3.99$ & $6.65$ & $13.30$ \\
$b$ & $1.752$ & $+1.997$ & $+4.976$ & $0.53$ & $0.88$ & $1.75$ \\
$c$ & $-18.460$ & $-21.044$ & $-52.426$ & $5.54$ & $9.23$ & $18.46$ \\
$d$ & $-15.200$ & $-17.328$ & $-43.168$ & $4.56$ & $7.60$ & $15.20$ \\

